On Zeno-like Behaviors in the Event Calculus with Goal-directed Answer Set Programming

It has been argued that Event Calculus (EC) is suitable for modeling high-level specifications of safety-critical cyber-physical systems. The primary advantage lies in the rather small semantic gap between EC models and requirements expressed in a semi-formal natural language. Moreover, its use of continuous time and variables avoids imprecision that stems from discretization. In the past, we have shown that a goal-directed ASP system can be used for implementing these EC models. However, precise representation of time as an infinitesimally divisible continuous quantity leads to Zeno-like behaviors and to non-termination in such a system. In this work, we model a number of well-known example problems from the literature to systematically study various natural EC modeling patterns that yield these Zeno-like behaviors, and propose ways to deal with them. Moreover, we also propose a technique to automatically detect all such cases.

==> eptcsdata.tex <==
\providecommand{\firstpage}{496}
\providecommand{\publicationstatus}{M. Gebser, D. Inclezan, F. Ricca, M. Carro \& M. Truszczynski:\\
41st International Conference on Logic Programming (ICLP 2025)\\
EPTCS 439, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.439.34}{10.4204/EPTCS.439.34}}
\pdfoutput=1

